Jev for Scientific Decisions: Evaluating Semantic Choices and Their Consequences

Scientific workflows often require choosing among known relations before a deterministic calculation can proceed. Whether observations share a culture, treatment or reference standard can change the scientific meaning of the resulting count or comparison. Once the evidence is prepared and the calculation is written as code, this decision reduces to selecting one of the listed candidates. We evaluate Jev on this step, using a harness that follows its documented guidance. The study compares twelve model configurations on ten scientific cases built from published sources. Each case contains two Choices, which are questions with listed candidates. Each case is repeated five times per configuration. We measure selections, downstream outputs and final labels separately. Jev tied with five other configurations at complete semantic correctness and achieved the lowest median latency and mean cost. On one Choice, whether samples came from one culture, three comparison configurations made seven wrong selections that changed downstream counts while preserving the correct final label. These results support using Jev to select relations when the evidence and candidates are prepared in advance. They also show that evaluating it requires checking the selections and downstream outputs that a workflow will reuse.

==> main_table_rows.tex <==
Jev 1.13 & 50 & 100 & 50 & 50 & --- & 0.335 & 0.442 & 0.0595\textsuperscript{a} \\
GPT-5.6 Luna & 50 & 99 & 49 & 50 & 32 & 1.509 & 2.753 & 0.2025\textsuperscript{b} \\
GPT-5.6 Terra & 49 & 98 & 49 & 49 & 0 & 1.166 & 2.147 & 1.5391\textsuperscript{b} \\
GPT-5.6 Sol & 50 & 100 & 50 & 50 & 0 & 1.385 & 2.370 & 3.0470\textsuperscript{b} \\
GPT-6 Astra & 50 & 100 & 50 & 50 & 0 & 2.384 & 4.418 & 7.6174\textsuperscript{b} \\
Claude Sonnet 5 & 50 & 100 & 50 & 50 & 0 & 2.162 & 5.422 & 4.2502\textsuperscript{b} \\
Claude Opus 5 & 50 & 100 & 50 & 50 & 0 & 3.237 & 3.967 & 10.6965\textsuperscript{b} \\
Qwen3.8 Flash & 42 & 83 & 41 & 42 & 636 & 14.182 & 34.320 & 0.4013\textsuperscript{a} \\
Qwen3.8 Max 0902 & 50 & 95 & 45 & 50 & 521 & 14.236 & 21.393 & 4.8302\textsuperscript{a} \\
DeepSeek V4.1 Flash & 48 & 96 & 48 & 48 & 370 & 5.449 & 8.821 & 0.3508\textsuperscript{a} \\
DeepSeek V4 Pro 0813 & 49 & 98 & 49 & 49 & 429 & 7.569 & 10.086 & 3.4299\textsuperscript{a} \\
Kimi K3 & 50 & 100 & 50 & 50 & 244 & 11.116 & 25.744 & 5.4663\textsuperscript{a} \\
